THERADIA WoZ: An Ecological Corpus for Appraisal-based Affect Research in Healthcare

We present THERADIA WoZ, an ecological corpus designed for audiovisual research on affect in healthcare. Two groups of senior individuals, consisting of 52 healthy participants and 9 individuals with Mild Cognitive Impairment (MCI), performed Computerised Cognitive Training (CCT) exercises while receiving support from a virtual assistant, tele-operated by a human in the role of a Wizard-of-Oz (WoZ). The audiovisual expressions produced by the participants were fully transcribed, and partially annotated based on dimensions derived from recent models of the appraisal theories, including novelty, intrinsic pleasantness, goal conduciveness, and coping. Additionally, the annotations included 23 affective labels drew from the literature of achievement affects. We present the protocols used for the data collection, transcription, and annotation, along with a detailed analysis of the annotated dimensions and labels. Baseline methods and results for their automatic prediction are also presented. The corpus aims to serve as a valuable resource for researchers in affective computing, and is made available to both industry and academia.

==> sections/Archived/3.Sota_emotion.tex <==
% \section{State of the art - Affective states}
% According to appraisal theories, affective phenomena are defined as multi-component processes aiming to maintain the well-being and survival of individuals in their environment \cite{FRIJDA04-EMO, SANDER13-MOD}. Roughly speaking, affective phenomena would arise when the meaning of environmental stimuli are - cognitively - appraised as potentially threatening to the equilibrium of individuals in their environment. This appraisal process would be divided into five criteria (themselves divided into sub-criteria, see \cite{SANDER05-CPM} for a detailed review): the relevance, which appraises how relevant the stimuli are for the individuals; the implication, which appraises the possible consequences of stimuli in relation to the individual's well-being and survival; the coping, which appraises the extent to which individuals can adapt or cope to these consequences; and the normative significance, which appraises whether the stimulus meaning is in line with the individual's norms and values. Following this appraisal process, the activation of organism's subsystems (i.e., physiological responses, action tendencies and motor expressions) would be synchronized to help individuals perform the adapted behaviors that can lead to the return of their homeostasis - or well-being and survival. This approach lies in the epistemological current of affectivism \cite{DUKES21-AFF} in which affective and non-affective phenomena do not differ in nature. The point is that all episodes of environmental interactions are ultimately governed by the quest to maintain homeostasis and likely involve activation of organism's subsystems. Thus, the distinction between affective and non-affective phenomena would be a matter of filling conditions (e.g., the trigger object, the degree of organism's subsystem synchronisation, the behavioral impact and the duration of the episode \cite{SCHERER05-WHAT,SCHERER05-UNCONSCIOUS}). In this perspective, affective state corresponds to a marker of how individuals appraise themselves between the plausible deregulation of their homeostasis caused by the environment and the search for the behavior leading to a return to equilibrium. 

% \subsection{The dimensional approach}
% One way of approximating the affective states of individuals is to think of them as points on a plane. Based on this approach, most of the literature have used the Circumplex to describe them, a Cartesian plane defined by two axes, namely valence (from unpleasant to pleasant) and arousal (from deactivation to activation) \cite{RUSSEL09-CORE, RUSSEL80-CIRCUM}. However, this approach drew a number of criticisms for its ability to differentiate affective states. On the one hand, valence should be seen as a multidimensional concept resulting from several dimensions \cite{FOURNIER22-COMB}. On the other hand, considering only two dimensions seems not sufficient to separate affective states. For instance, fear and anger are both defined by high arousal and negative valence. Thus, authors stated that at least four dimensions should be taken into account to appropriately distinguish affective states \cite{FONTAINE07-DIM}.

% According to appraisal theories, the cognitive appraisal process would be causal in the elicitation of affective episodes \cite{MOORS13-CAUSAL}. This position assumes a necessary and sufficient relationship would link appraisal to the synchronization of organism's subsystems \cite{SIEMER07-NECESS}. In other words, a specific pattern of criteria of the appraisal process would trigger a specific synchronized activation of organism's subsystems. Conversely, the observation of a specific synchronized activation would allow to predict the pattern of criteria of the appraisal process performed by the experimenter of the affective episode. Based on these premises, the Tripartite Emotion Expression and Perception (TEEP) model \cite{SCHERER19-TEEP} postulates that the way humans perceive affect of others is conditioned by this causal relationship. The idea is that if an individual A is able to determine the affective state of an individual B, this is because A inferred (in part unconsciously) the cognitive appraisal process performed by B on the basis of the motor expressions (e.g., facial expression) that B has produced. In brief, appraisal theories proposes to solve the problem of affective state differentiation based on a n-dimensional hyperplane representing the criteria (or sub-criteria) of the appraisal process. 

% \subsection{The categorical approach}
% Labels are another common way of approximating individual's affective states. Appraisal theories suggest that the use of labels represents a way for humans to characterize the conscious part of the activation states of the organism's subsystems (i.e., of cognitive appraisal process, physiological responses, action tendencies, and motor expressions) \cite{GRANDJEAN08-CONSCIOUS, MOORS14-FLAVOR}. Thus, this assumes that each affective label would represent a specific pattern of criteria of the appraisal process \cite{SCHERER19-TEEP, SCHERER13-APPLAB, SCHERER18-EMOTINFER}. One of the crucial points of such an approach is to select affective labels likely to be relevant in the context of interest. While basic emotion labels (i.e., anger, fear, sadness, happiness, disgust, see \cite{TRACY11-BASIC} for details) are commonly used to model affective states, they do not seem appropriate to the context of healthcare and AI-patients interactions. In the case of CCT in which patients are involved in exercise achievement while being assisted by a "coach" (whether a therapist or potential AI technology), it seems fair to expect that affects more complex than basic emotions will be experienced. That said, this case study seems to correspond strongly to that of the school environment, in which students are also involved in carrying out exercises assisted by a coach, namely the teacher. In the literature, the theoretical framework of achievement emotions has been developed to account for relevant affects in the educational environment. 



% - Blend emotions 




==> sections/Archived/6.Annotations.tex <==
% \section{Collection of annotations}
% •	Annotations tool
% •	Annotation guidelines
% •	Annotation data collection

% \begin{figure}[!t]
% \centering
% \includegraphics[width=2.5in]{Computer_Society_LaTeX_template/plots/plot_annot.png}
% \caption{Example of annotated extract  based on intrinsic pleasantness}
% \label{fig_1}
% \end{figure}

% •	Post-processing


==> sections/Archived/7.Annotations_analysis.tex <==
% \section{Analysis of annotations}



% \subsection{Categorical annotations}
% For each sequence, an annotator could choose an arbitrary number of emotions, and then was asked to give a number (between zero and 100) corresponding to the intensity of the observed emotion. Therefore, we assume that the intensity of the emotions that were not chosen for a given annotator to be zero. This leaves us with numerical vectors that represent the intensity of each emotion for each sequence and each annotator. 

% \subsubsection{The frequency of categories}
% To evaluate how frequent each emotion category was present in each sequence, we simply count the number of sequences, where a given category was chosen by at least one annotator. Furthermore, we also counted the number of sequences, where a given category was chosen by at least two, three, or four annotators. The results are put in Figure \ref{fig:freq_labels}.

% \begin{figure}[!ht]
% %\centering
% \includegraphics[width=0.48\textwidth]{Computer_Society_LaTeX_template/plots/freq_labels.png}
% \caption{The frequency of the existence of each emotion category for each sequence if at least one, two, three, or four annotators have chosen the emotion category. Note that the vertical axis is on a logarithmic scale for visual purposes.}
% \label{fig:freq_labels}
% \end{figure}

% \subsubsection{Inter-Annotator Agreement}

% As mentioned above, each emotion category first had to be chosen, and then given a value between zero to 100 based on the perceived intensity of emotion. Therefore, here we calculate the inter-annotator agreement for both the existence of an emotion, and the estimated intensities. The two cases are explained in more detail below and the results are provided in Table \ref{tab:coreset-overview}.

% \subsubsection{Agreement on the existence of emotion}

% To calculate the inter-annotator agreement of the existence of emotion, we chose the Unweighted Average Recall (UAR) metric, which can be described as below:

% \begin{equation}
%     UAR = \frac{1}{k} \sum_{i=1}^k \frac{N_c^i}{N^i}
%     \label{UAR}
% \end{equation}

% where k is the total number of classes, $N_c^i$ and $N^i$ are the number of correctly identified instances and the total number of instances for class $i$ respectively. Note that if the number of instances in different classes is balanced, then the UAR is equal to the accuracy. Therefore, UAR has also been mentioned in the literature as "weighted accuracy".


% We also looked at Cohen's kappa to calculate the inter-annotator agreement on the presence of emotion. However, the original Cohen's kappa formula is based on the assumption that an annotator has to choose a label from a set of labels. This is not the case here, as each annotator can choose (or not choose) any emotion label. Further attempts to make Cohen's kappa work on a range were also unsuccessful, as this would result in a bias of many zero values for the emotions that were not selected.


% \subsubsection{Agreement on the intensity of emotion}

% In this case, we simply used Pearson's correlation because it is a common metric for calculating inter-annotator agreement for two sets of continuous values.

% \subsubsection{Relation between Appraisals and Emotions}

% \subsection{Continuous dimensional annotations}

% \begin{table}[ht!]
% \setlength{\tabcolsep}{7pt}
% \renewcommand{\arraystretch}{1.5}
% \footnotesize
% \caption{Inter-Annotator Agreement based on the concordance correlation coefficient for continuous appraisal dimensions and dimensions summaries (averaged over sequences)}
% \label{tab:agreement_dim}
% \tiny
% \begin{tabular}{llllll}
% \hline
%  & \textbf{Arousal} & \textbf{Coping}& \textbf{Novelty} & \textbf{\begin{tabular}[c]{@{}l@{}}  Intrinsic\\ pleasantness\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Goal\\ conduciveness\end{tabular}} \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Continuous\\ dimensions\end{tabular}} 
% & 0.23 $\pm$ 0.17  & \begin{tabular}[c]{@{}l@{}}0.28 $\pm $ 0.21
% \end{tabular} & 0.13 $\pm$ 0.17  & 0.24 $\pm$ 0.21  & 0.29 $\pm$ 0.21 \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Dimensions\\ summaries\end{tabular}} & 0.10 $\pm$ 0.05  & 0.59 $\pm$ 0.10  & 0.28 $\pm$ 0.18  & 0.59 $\pm$ 0.08 & 0.55 $\pm$ 0.10     \\ \hline
% \end{tabular}
% \end{table}

% %We calculate agreement between annotators through multiple measures. 
% For continuous appraisal dimensions, we use the 
% concordance correlation coefficient (CCC) \cite{ccc} as a metric to compare the ratings of two annotators. The CCC for two vectors $x$ and $y$ is: 
% \begin{equation}
% CCC(x, y)=\frac{2 \rho \sigma_x \sigma_y}{\sigma_x^2+\sigma_y^2+\left(\mu_x-\mu_y\right)^2}
% \end{equation}
% where $\rho$ is the (Pearson’s) correlation coefficient, $\mu_x$ and $\mu_y$ are the means for the vectors $x$ and $y$ respectively and their variances are defined as $\sigma_x$ and $\sigma_y$.
% Table \ref{tab:agreement_dim} shows the mean and std values of the obtained CCC between annotators for each dimension across all sequences.

% \subsection{Summarised dimensional annotations}

% \begin{figure*}[t]
% \centering
% \captionsetup{justification=centering}
% \includegraphics[width=\textwidth]{Computer_Society_LaTeX_template/plots/dist-dim.png} 
% \caption{ Distributions of appraisal dimensions of each annotator}
% \label{fig:Name}
% \end{figure*}



==> sections/Archived/8.CoreSet.tex <==
% \section{Label core set selection}
% •	Summary table (All labels in rows and all analyses in columns then add a cross for labels meeting the analysis selection criteria)
% •	Add a table for each analysis
% •	e.g., CCC
% •	e.g., label - dimension

% \input{Computer_Society_LaTeX_template/tables/coreset_overview}

% \subsection{Relation between Appraisals and Emotions}

% \begin{figure}[t]
% %\centering
% \includegraphics[width=0.48\textwidth]{Computer_Society_LaTeX_template/plots/corr_emotions_dim/all_users.png}
% \caption{Heatmaps showing Pearson’s correlation coefficients between appraisals (on the columns) and emotions (on the rows) for the six annotators. Significant correlations (p-value $\leq{0.05} $) are colored either in red (positive) or blue (negative). While nonsignificant correlations (p-value$>0.05$) are presented with 0 shown in grey.}
% \label{fig_2}
% \end{figure}


% In this section, we investigate the relationship between appraisal and emotions to perform the label core set analysis. Figure \ref{fig_2} shows the correlation heatmaps of appraisals across emotions from the ratings provided by each annotator. 

% Each cell reports the Pearson correlation coefficient between the averaged appraisal dimension values over a given sequence (on the columns) with a given emotion (on the rows). Dense colors and high numbers indicate that the appraisal dimension and emotion in question are strongly related, while light colors and low values show a weak relationship. For instance, for the first annotator, a high degree of arousal and novelty is related to a strong excitement more than to other emotions. While low degrees of coping, goal conduciveness and intrinsic pleasantness is associated with frustration, disappointment, separation, anxiety,  nervousness and anger. However, no significant correlation was obtained between the five appraisal dimensions and sadness, guilt, curiosity, interest, patience and contemptuousness. This shows that according to this annotator's experience, this set of emotions does not indicate any motivational relevance or significance with situations related to appraisals dimensions considered in this context. 

% In order to understand the commonly experienced types of emotions with respect to appraisal dimensions, we compare the obtained correlation matrices of the six annotators. Our hypothesis relies on the fact that agreement in the obtained associations between the annotator's ratings could be of help to identify the set of emotions showing a significant affective experience. \todosaf{TODO: maybe we need to add some refs in line with past studies in psychology}. Therefore based on this hypothesis, we selected the set of emotions to omit to be the emotions where at least two annotators show a nonsignificant correlation with appraisal dimensions as the following: disappointed, sad, embarrassed, guilty, upset, nervous, impatient, comptempous, ashamed, curious, proud, excited. \todosaf{TBC}



==> tables/ASR.tex <==
\begin{table*}[ht!]
\small
%\tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, \Huge
  \caption{Automatic Speech Recognition (ASR) results on all the transcribed sequences, where there exists text based on human transcription. The results are mean (std) of Word Error Rate (WER) for all sequences according to different ASR models}
  \label{tab:ASR}
  \centering
  
  \begin{tabulary}{1.0\textwidth}{m{0.1\textwidth}|M{0.07\textwidth}M{0.07\textwidth}M{0.07\textwidth}|M{0.07\textwidth}M{0.07\textwidth}M{0.07\textwidth}|M{0.07\textwidth}M{0.07\textwidth}M{0.07\textwidth}}

\hline
 \multirow{2}{*}{ASR model} & \multicolumn{3}{c|}{Senior} & \multicolumn{3}{c|}{MCI} & \multicolumn{3}{c}{Senior + MCI} \\
 \cline{2-10}
 & Emotional & Neutral & All & Emotional & Neutral & All & Emotional & Neutral & All \\
 \hline
Google & 55.45\% (43.40\%) & 49.48\% (44.96\%) & 54.15\% (43.82\%) & 49.56\% (39.83\%) & 46.72\% (43.98\%) & 47.80\% (42.45\%) & 55.22\% (43.28\%) & 48.95\% (44.78\%) & 53.65\% (43.74\%) \\
 \hline
Vosk-small & 57.79\% (43.97\%) & 52.60\% (44.84\%) & 56.65\% (44.21\%) & 48.67\% (39.45\%) & 40.33\% (41.51\%) & 43.50\% (40.92\%) & 57.43\% (43.83\%) & 50.23\% (44.47\%) & 55.63\% (44.10\%) \\
 \hline
Vosk-medium & 48.00\% (49.05\%) & 38.49\% (45.49\%) & 45.92\% (48.45\%) & 39.82\% (42.72\%) & 29.04\% (39.60\%) & 33.14\% (41.12\%) & 47.68\% (48.84\%) & 36.67\% (44.57\%) & 44.92\% (48.04\%) \\
 \hline
Vosk-linto & 56.51\% (44.66\%) & 50.90\% (44.94\%) & 55.28\% (44.78\%) & 49.10\% (39.42\%) & 40.04\% (41.12\%) & 43.48\% (40.70\%) & 56.21\% (44.49\%) & 48.81\% (44.43\%) & 54.36\% (44.58\%) \\
 \hline
Frequency & 7859 & 2201 & 10060 & 322 & 526 & 848 & 8181 & 2727 & 10908 \\
 \hline
Word / second & .791 (.624) & .719 (.563) & .775 (.611) & .877 (.641) & .748 (.601) & .797 (.620) & .794 (.625) & .725 (.570) & .777 (.612) \\
\hline
        
\end{tabulary}
\end{table*}

==> tables/ASR_emo.tex <==
\begin{table}[t!]
\scriptsize
%\tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, \Huge
  \caption{The results for affective label intensity prediction for human vs automatic transcriptions (Google's ASR).}
  \label{tab:asr-emo}
  \centering
  \begin{tabulary}{1.0\textwidth}{m{0.07\textwidth}|R{0.04\textwidth}R{0.04\textwidth}|R{0.04\textwidth}R{0.04\textwidth}}

\hline
\multirow{2}{*}{Label} & \multicolumn{2}{c|}{TF-IDF} & \multicolumn{2}{c}{BERT}  \\
 & \multicolumn{1}{c}{Human} & \multicolumn{1}{c|}{Automatic} & \multicolumn{1}{c}{Human} & \multicolumn{1}{c}{Automatic}  \\
\hline
Annoyed & .031 & .075 & .122 & .255 \\
Anxious & .140 & .115 & .124 & .087 \\
Confident & .263 & .233 & .518 & .473 \\
Desperate & .211 & .172 & .322 & .221 \\
Frustrated & .381 & .327 & .183 & .222 \\
Happy & .127 & .117 & .157 & .108 \\
Interested & .156 & .147 & .336 & .364 \\
Relaxed & .341 & .314 & .295 & .363 \\
Satisfied & .344 & .323 & .364 & .057 \\
Surprised & .209 & .167 & .197 & .143 \\ 
\hline
Average & .220 & .199 & .262 & .229  \\
\hline



  \end{tabulary}
\end{table}

==> tables/Archived_table/Induction_table.tex <==
\begin{table}[t!]
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.5}
\footnotesize
\caption{Types of induction assigned to the different groups according to exercise introduction, difficulty and feedback.}
\label{tab:induction-overview}
\begin{tabular}{lllll}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Participant\\ group\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Task\\ number\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Exercise introduction\\ induction\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Real difficulty\\ of the exercise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Feedback\\ induction\end{tabular}}\\ \hline
\text{A} & 2  & Easy & Easy & Congratulation\\
\text{A} & 4  & Easy & Hard & Critical +\\
\text{A} & 6  & Hard & Easy & Critical\\
\text{A} & 8  & Hard & Hard & Congratulation +\\
\text{B} & 2  & Easy & Easy & Congratulation +\\
\text{B} & 4  & Easy & Hard & Congratulation\\
\text{B} & 6  & Hard & Easy & Critical +\\
\text{B} & 8  & Hard & Hard & Critical\\
\text{C} & 2  & Easy & Easy & Critical\\
\text{C} & 4  & Easy & Hard & Congratulation +\\
\text{C} & 6  & Hard & Easy & Congratulation\\
\text{C} & 8  & Hard & Hard & Critical +\\
\text{D} & 2  & Easy & Easy & Critical +\\
\text{D} & 4  & Easy & Hard & Critical\\
\text{D} & 6  & Hard & Easy & Congratulation +\\
\text{D} & 8  & Hard & Hard & Congratulation\\ \hline
\end{tabular}
\end{table}

==> tables/Archived_table/cognitive_delay.tex <==
\begin{table}[t!]
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.5}
\scriptsize
\caption{Cognitive delay in continuous annotation as a function of dimensions}
\label{tab:cognitive_delay}
\begin{tabular}{cccccc}
\hline
 & \textbf{Arousal} & \textbf{Novelty}& \textbf{\begin{tabular}[c]{@{}c@{}}  Intrinsic\\ pleasantness\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Goal\\ conduciveness\end{tabular}} & \textbf{Coping} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Number of \\extracts\end{tabular}} 
& 4 & \begin{tabular}[c]{@{}l@{}} 6
\end{tabular} & 5 & 5  & 7\\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Cognitive \\delay (ms)\end{tabular}} & 1.99 $\pm$ 0.43  & 1.32 $\pm$ 0.51  & 1.13 $\pm$ 0.36  & 3.30 $\pm$ 0.65 & 1.33 $\pm$ 0.48     \\ \hline
\end{tabular}
\end{table}

==> tables/bias_dim.tex <==
\begin{table*}[ht!]
\centering
\caption{The bias and fairness analysis of the multi-modal dimension regression models. The reported results are in Concordance Correlation Coefficients (CCC).}
\label{bias_dim}
\setlength{\tabcolsep}{6pt}
% \renewcommand{\arraystretch}{1.8}
\small
\begin{tabular}{l|ccccc|ccccc}
\hline
\multirow{3}{*}{Dimensions}& \multicolumn{5}{c|}{Time-continous}& \multicolumn{5}{c}{Summaries}\\ \cline{2-11} 
\multicolumn{1}{c|}{\multirow{2}{*}{}} & \multicolumn{3}{c}{Senior}& \multirow{2}{*}{MCI} & \multicolumn{1}{c|}{\multirow{2}{*}{Senior+MCI}} & \multicolumn{3}{c}{Senior} & \multirow{2}{*}{MCI} & \multirow{2}{*}{Senior+MCI} \\ %\cline{2-11} 
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c}{Female} & \multicolumn{1}{c}{Male} & \multicolumn{1}{c}{F+M} & \multicolumn{1}{c}{}    & \multicolumn{1}{c|}{}           & \multicolumn{1}{c}{Female} & \multicolumn{1}{c}{Male} & \multicolumn{1}{c}{F+M} & \multicolumn{1}{c}{}    & \multicolumn{1}{c}{}           \\ \hline
Arousal& .626& .577& .614& .713& .624& .280& .361& .315& .360& .310\\ %\hline
Coping& .458& .350& .433& .530& .442& .690& .608& .674& .799& .684\\ %\hline
Goal conduciveness& .472& .312& .434& .529& .444& .668& .610& .658& .711& .662\\ %\hline
Intrinsic pleasantness& .466& .269& .420& .562& .434& .634& .448& .598& .709& .609\\ %\hline
Novelty& .354& .249& .330& .387& .335& .607& .348& .543& .709& .559\\ \hline
\end{tabular}
\end{table*}

==> tables/bias_dim_c.tex <==
\iffalse
\begin{table}[ht!]
\centering
\caption{The bias and fairness analysis of the multi-modal continuous dimension regression models. The reported results are in Concordance Correlation Coefficients (CCC).}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.8}
\scriptsize
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{c}{} &        & \multicolumn{3}{c}{Senior}              & \multicolumn{1}{c}{\multirow{2}{*}{MCI}} & \multicolumn{1}{c}{\multirow{2}{*}{Senior+MCI}} \\ \cline{1-5}
Dimension           & GS     & \multicolumn{1}{c}{Female} & \multicolumn{1}{c}{Male} & \multicolumn{1}{c}{All} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}        \\ \hline

\multirow{3}{*}{Arousal}& Mean   & .581   & .492 & .560 & .750 & .579\\ \cline{2-7} 
& Median & .673   & .659& .669 & .807& .683\\ \cline{2-7} 
& EWE    & .626   & .577& .614 & .713& .624\\ \hline

\multirow{3}{*}{Coping} & Mean   & .395   & .303 & .374 & .460 & .382    \\ \cline{2-7} 
& Median & .349   & .275& .332& .413& .340\\ \cline{2-7} 
& EWE    & .458   & .350& .433 & .530& .442    \\ \hline

\multirow{3}{*}{Goal conductiveness}    & Mean   & .416   & .276 & .383 & .435 & .388    \\ \cline{2-7} 
 & Median & .373   & .305 & .357 & .424 & .364    \\ \cline{2-7} 
 & EWE    & .472   & .312 & .434 & .529 & .444    \\ \hline

\multirow{3}{*}{Intrinsic pleasantness} & Mean   & .386   & .208 & .345 & .472 & .358    \\ \cline{2-7} 
 & Median & .339   & .296 & .329 & .450 & .341    \\ \cline{2-7} 
 & EWE    & .466   & .269 & .420 & .562 & .434    \\ \hline

\multirow{3}{*}{Novelty}  & Mean   & .336   & .235 & .312 & .418 & .323    \\ \cline{2-7} 
 & Median & .290   & .151 & .258 & .398 & .272    \\ \cline{2-7} 
 & EWE    & .354   & .249 & .330 & .387 & .335    \\ \hline
\end{tabular}
\end{table}
\fi

==> tables/bias_dim_s.tex <==
\iffalse
\begin{table*}[ht!]
\centering
\caption{The bias and fairness analysis of the multi-modal dimension summaries regression models. The reported results are in Concordance Correlation Coefficients (CCC).}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.8}
\scriptsize
\begin{tabular}{llllllllllll}
\hline
&& \multicolumn{5}{c}{Traditional features}& \multicolumn{5}{c}{Deep representations}\\ \hline
\multicolumn{1}{c}{}&& \multicolumn{3}{c}{Senior}& \multicolumn{1}{c}{\multirow{2}{*}{MCI}} & \multicolumn{1}{c}{\multirow{2}{*}{Senior+MCI}} & \multicolumn{3}{c}{Senior}& \multicolumn{1}{c}{\multirow{2}{*}{MCI}} & \multicolumn{1}{c}{\multirow{2}{*}{Senior+MCI}} \\ \cline{1-5} \cline{8-10}
Dimension& GS& \multicolumn{1}{c}{Female} & \multicolumn{1}{c}{Male} & \multicolumn{1}{c}{All} & \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}& \multicolumn{1}{c}{Female} & \multicolumn{1}{c}{Male} & \multicolumn{1}{c}{All} & \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}\\ \hline
\multirow{2}{*}{Arousal}& Mean   & .365& .265& .346& .538& .365& .280& .361& .315& .360& .310\\ \cline{2-12} 
& Median & .353& .304& .351& .430& .360& .276& .321& .301& .313& .305\\ \hline
\multirow{2}{*}{Coping}& Mean   & .647& .610& .445& .742& .621& .690& .608& .674& .799& .684\\ \cline{2-12} 
& Median & .640& .447& .607& .770& .621& .672& .595& .658& .802& .669\\ \hline
\multirow{2}{*}{Goal conductiveness}    & Mean   & .660& .506& .635& .752& .647& .668& .610& .658& .711& .662\\ \cline{2-12} 
& Median & .635& .486& .613& .710& .623& .644& .607& .638& .709& .644\\ \hline
\multirow{2}{*}{Intrinsic pleasantness} & Mean   & .595& .433& .576& .749& .595& .634& .448& .598& .709& .609\\ \cline{2-12} 
& Median & .574& .426& .555& .695& .570& .635& .498& .609& .616& .608\\ \hline
\multirow{2}{*}{Novelty}& Mean   & .556& .247& .475& .675& .493& .607& .348& .543& .709& .559\\ \cline{2-12} 
& Median & .461& .165& .375& .661& .395& .500& .268& .436& .628& .453\\ \hline
\end{tabular}
\end{table*}
\fi

==> tables/dim_c_coef.tex <==
\begin{table}[ht!]
\caption{The coefficients learned by the GRU model per each modality for decision fusion for continuous dimension prediction}
\label{weigh_dimc}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.5}
\small
\centering
\begin{tabular}{llll}
\hline
& \multicolumn{3}{c}{Modalities}\\ \hline
GS& \multicolumn{1}{c}{Text}     & \multicolumn{1}{c}{Audio}    & \multicolumn{1}{c}{Video}    \\ \hline
Mean& \multicolumn{1}{r}{33.51 \%} & \multicolumn{1}{r}{33.57 \%} & \multicolumn{1}{r}{32.91 \%} \\ \hline
Median& 29.24 \%& 39.00 \%& 31.75 \%\\ \hline
\multicolumn{1}{l}{EWE} & 31.74 \%& 35.97 \%& 32.27 \%\\ \hline
\end{tabular}
\end{table}

==> tables/dim_s_coef.tex <==
\iffalse
\begin{table}[t!]
\centering
\caption{The coefficients of the linear regression model per each modality for decision fusion of traditional and deep representations for dimension summaries prediction}

\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.5}
\scriptsize
\begin{tabular}{ccccclcc}
\hline
& &  & & Modalities & & &        \\ \hline
& & \multicolumn{2}{c}{A}      & \multicolumn{2}{c}{T}       & \multicolumn{2}{c}{V} \\ \hline
Dimensions & GS & Trad.F & Deep.F & Trad.F & \multicolumn{1}{c}{Deep.F} & Trad.F    & Deep.F    \\ \hline
\multirow{2}{*}{Arousal} & Mean   & \multicolumn{1}{l}{9 \%} & \multicolumn{1}{l}{46.18 \%} & \multicolumn{1}{l}{76.00 \%} & 35.17 \%& 23.05 \% & 17.78\%     \\ \cline{2-8} 
 & Median & -2.96 \%& 47.72 \% & 74.22 \%& 41.09\%& 28.74 \% & 17.02 \%    \\ \hline
\multirow{2}{*}{Coping}      & Mean   & 4\% & 49.95 \%      &73.78 \%& 45.06 \%& 22.20 \% & 33.92 \%   \\ \cline{2-8} 
 & Median &3.07 \%& 44.53 \% &67.84 \%& 45.99 \%& 29.07\% & 38.54 \%    \\ \hline
\multirow{2}{*}{Goal conductiveness}  & Mean   & 3.12 \%& 51.41 \%     &67.72 \%& 53.41 \%&  29.15 \%   & 31.79 \%     \\ \cline{2-8} 
& Median & 1.82 \%& 50.54 \% & 70.36 \%& 49.26 \%& 27.81 \% & 36.01 \%   \\ \hline
\multirow{2}{*}{Intrinsic pleasantness} & Mean   & 0.02 \%& 50.16 \%& 65.05 \%& 38.41 \%& 34.92 \%& 36.43  \%  \\ \cline{2-8} 
& Median & -0.090 \% & 41.44 \% & 66.58 \% & 45.33 \%& 33.50 \% & 38.10 \%    \\ \hline
\multirow{2}{*}{Novelty} & Mean   &8.87 \% & 52.77 \% & 70.91 \% & 53.02 \%& 20.21 \%& 16.39 \%     \\ \cline{2-8} 
& Median &7.93 \% & 52.09 \%& 75.70 \%& 61.39 \%& 16.36 \%& 13.35 \%    \\ \hline
\end{tabular}
\end{table}
\fi

\begin{table}[t!]
\centering
\caption{The coefficients (\%) of the linear regression model per each modality for decision fusion of traditional and deep representations for dimension summaries prediction}
\label{coef_s}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.5}
\scriptsize
\begin{tabular}{clrlrlrl}
\hline
& & \multicolumn{6}{c}{Modalities} \\ \hline
 & & \multicolumn{2}{c}{Text} & \multicolumn{2}{c}{Audio}    & \multicolumn{2}{c}{Video} \\ \hline
Dimensions & GS     & \multicolumn{1}{c}{TF-IDF} & \multicolumn{1}{c}{BERT} & \multicolumn{1}{c}{MFB} & \multicolumn{1}{c}{W2V2} & \multicolumn{1}{c}{FAU} & \multicolumn{1}{c}{CLIP} \\ \hline

\multirow{2}{*}{Arousal}        & Mean   & 71.91 & 39.67     & 1.56 & 43.95     & 26.53    & 16.36     \\ \cline{2-8} 
 & Median & 70.31& 44.29     & 0.61     & 41.48     & 29.08    & 14.22     \\ \hline

\multirow{2}{*}{Coping}      & Mean   & 69.48& 35.05     & 3.86     & 35.73     & 26.66    & 26.33     \\ \cline{2-8} 
& Median & 63.81& 29.92     & 3.66     & 36.88     & 32.53    & 33.19     \\ \hline

\multirow{2}{*}{Goal conduciveness}    & Mean   & 64.62& 38.63     & 2.87     & 37.22     & 32.51    & 24.14     \\ \cline{2-8} 
& Median & 66.99& 35.63     & 1.52     & 37.15     & 31.49    & 27.21     \\ \hline

\multirow{2}{*}{Intrinsic pleasantness} & Mean   & 62.20& 36.06     & -0.06    & 26.28     & 37.86    & 27.65     \\ \cline{2-8} 
& Median & 63.86& 25.99     & -0.24    & 41.48     & 36.37    & 32.52     \\ \hline

\multirow{2}{*}{Novelty}        & Mean   & 70.14& 30.64     & 7.68     & 50.38     & 22.17    & 18.96     \\ \cline{2-8} 
& Median & 75.21& 32.79     & 8.01     & 52.87     & 16.78    & 18.09     \\ \hline
\end{tabular}
\end{table}


==> tables/dim_sum.tex <==
\begin{table*}[t]
\small
%\tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, \Huge
  \caption{The results for the dimensional summary in CCC. \textbf{Trying linear with Tanh, as the outputs seem correlated but somehow not on the same scale, that seems to be why multi-modal is fine}}
  \label{tab:dim-summary}
  \centering
  
  \begin{tabulary}{1.0\textwidth}{m{0.15\textwidth}|R{0.04\textwidth}R{0.04\textwidth}R{0.04\textwidth}R{0.06\textwidth}|R{0.04\textwidth}R{0.04\textwidth}R{0.04\textwidth}R{0.06\textwidth}}

  \multirow{3}{*}{Dimension} & \multicolumn{4}{c|}{Traditional Features} & \multicolumn{4}{c}{Deep Representations} \\ \cline{2-9}
 & \multicolumn{1}{c}{Text} & \multicolumn{1}{c}{Audio} & \multicolumn{1}{c}{Video} & \multicolumn{1}{c|}{\multirow{2}{*}{Multi-modal}} & \multicolumn{1}{c}{Text} & \multicolumn{1}{c}{Audio} & \multicolumn{1}{c}{Video} & \multicolumn{1}{c}{\multirow{2}{*}{Multi-modal}} \\ %\cline{2-4} \cline{6-8}
 & \multicolumn{1}{c}{TF-IDF} & \multicolumn{1}{c}{MFB} & \multicolumn{1}{c}{FAU} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{BERT} & \multicolumn{1}{c}{W2V2} & \multicolumn{1}{c}{CLIP} & \multicolumn{1}{c}{} \\ \cline{1-9}

arousal & .187 & -.044 & .024 & .384 & -.020 & -.030 & .011 & .430 \\
coping & .426 & -.099 & .297 & .589 & -.029 & .096 & .411 & .636 \\
goal conduciveness & .451 & -.078 & .278 & .607 & -.029 & .079 & .365 & .643 \\
intrinsic pleasantness & .335 & -.086 & .272 & .598 & -.025 & .041 & .342 & .582 \\
novelty & -.184 & .064 & -.040 & .439 & .036 & .077 & .223 & .538 \\
\hline
average & .243 & -.049 & .166 & .523 & -.014 & .053 & .270 & .566 \\
        
  \end{tabulary}
\end{table*}

==> tables/dimensions_agr.tex <==

\begin{table}[ht!]
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.5}
\footnotesize
\caption{Inter-Annotator Agreement based on the concordance correlation coefficient for continuous appraisal dimensions and dimensions summaries (averaged over sequences)}
\label{tab:agreement_dim}
\tiny
\begin{tabular}{llllll}
\hline
 & \textbf{Arousal} & \textbf{Coping}& \textbf{Novelty} & \textbf{\begin{tabular}[c]{@{}l@{}}  Intrinsic\\ pleasantness\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Goal\\ conduciveness\end{tabular}} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Continuous\\ dimensions\end{tabular}} 
& 0.23 $\pm$ 0.17  & \begin{tabular}[c]{@{}l@{}}0.28 $\pm $ 0.21
\end{tabular} & 0.13 $\pm$ 0.17  & 0.24 $\pm$ 0.21  & 0.29 $\pm$ 0.21 \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Dimensions\\ summaries\end{tabular}} & 0.10 $\pm$ 0.05  & 0.59 $\pm$ 0.10  & 0.28 $\pm$ 0.18  & 0.59 $\pm$ 0.08 & 0.55 $\pm$ 0.10     \\ \hline
\end{tabular}
\end{table}




==> tables/label_cls_annots.tex <==
\begin{table*}[t]
\small
%\tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, \Huge
  \caption{The results of the traditional multimodal representations, according to which an emotion is present if at least one, two or three annotators have annotated a sequence.}
  \label{tab:label-cls-annots}
  \centering
  
  \begin{tabulary}{1.0\textwidth}{m{0.07\textwidth}|R{0.08\textwidth}R{0.08\textwidth}R{0.08\textwidth}|R{0.08\textwidth}R{0.08\textwidth}R{0.08\textwidth}}

  % \multirow{3}{*}{Label} & \multicolumn{3}{c|}{Traditional Features} & \multicolumn{3}{c}{Deep Representations} \\ \cline{2-7}

\hline
 \multirow{3}{*}{Label} & \multicolumn{3}{c}{Traditional Features} & \multicolumn{3}{c}{Deep Representations} \\ 
 \cline{2-7}

 & \multicolumn{6}{c}{Label existence prediction if it is annotated by by at least:} \\
  
 & \multicolumn{1}{c}{One annotator} & \multicolumn{1}{c}{Two annotators} & \multicolumn{1}{c}{Three annotators} & \multicolumn{1}{c}{One annotator} & \multicolumn{1}{c}{Two annotators} & \multicolumn{1}{c}{Three annotators} \\ %\cline{2-4} \cline{6-8}
\hline
Annoyed & 63.20\,\% & 67.33\,\% & 50.00\,\% & 63.33\,\% & 67.96\,\% & 71.80\,\% \\
Anxious & 62.87\,\% & 59.30\,\% & 66.86\,\% & 64.30\,\% & 65.83\,\% & 66.47\,\% \\
Confident & 70.88\,\% & 70.19\,\% & 71.15\,\% & 71.95\,\% & 74.80\,\% & 75.79\,\% \\
Desperate & 74.20\,\% & 69.11\,\% & 67.89\,\% & 72.07\,\% & 67.74\,\% & 64.27\,\% \\
Frustrated & 71.48\,\% & 68.89\,\% & 63.80\,\% & 70.32\,\% & 73.45\,\% & 73.17\,\% \\
Happy & 75.50\,\% & 74.21\,\% & 72.19\,\% & 68.41\,\% & 68.85\,\% & 63.58\,\% \\
Interested & 61.24\,\% & 60.75\,\% & 64.40\,\% & 63.05\,\% & 61.63\,\% & 64.60\,\% \\
Relaxed & 70.29\,\% & 74.53\,\% & 70.82\,\% & 73.05\,\% & 74.52\,\% & 68.81\,\% \\
Satisfied & 74.45\,\% & 70.93\,\% & 69.23\,\% & 72.29\,\% & 70.49\,\% & 68.92\,\% \\
Surprised & 60.19\,\% & 64.85\,\% & 61.63\,\% & 63.36\,\% & 67.93\,\% & 62.70\,\% \\
\hline
Average & 68.43\,\% & 68.01\,\% & 65.80\,\% & 68.21\,\% & 69.32\,\% & 68.01\,\% \\
\hline

  \end{tabulary}
\end{table*}

==> tables/label_reg_bias.tex <==
\begin{table*}[t]
\small
%\tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, \Huge
  \caption{The bias and fairness analysis of the multi-modal emotion regression models. The reported results are in Concordance Correlation Coefficients (CCC).}
  \label{tab:label-regression-bias}
  \centering
  
  \begin{tabulary}{1.0\textwidth}{m{0.07\textwidth}|M{0.05\textwidth}M{0.05\textwidth}M{0.05\textwidth}M{0.05\textwidth}M{0.08\textwidth}|M{0.06\textwidth}M{0.05\textwidth}M{0.05\textwidth}M{0.05\textwidth}M{0.08\textwidth}}

\hline
\multicolumn{1}{l|}{\multirow{3}{*}{Label}} & \multicolumn{5}{c|}{Traditional features} & \multicolumn{5}{c}{Deep representations} \\ \cline{2-11}

\multicolumn{1}{c|}{} & \multicolumn{3}{c}{Senior} & \multicolumn{1}{c}{\multirow{2}{*}{MCI}} & \multicolumn{1}{c|}{\multirow{2}{*}{Senior+MCI}} & \multicolumn{3}{c}{Senior} & \multicolumn{1}{c}{\multirow{2}{*}{MCI}} & \multicolumn{1}{c}{\multirow{2}{*}{Senior+MCI}} \\ %\cline{2-4} \cline{7-9}

\multicolumn{1}{c|}{} & \multicolumn{1}{c}{Female} & \multicolumn{1}{c}{Male} & \multicolumn{1}{c}{F+M} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{Female} & \multicolumn{1}{c}{Male} & \multicolumn{1}{c}{F+M} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\


\hline
Annoyed & .210 & .131 & .247 & .367 & .255 & .302 & .199 & .284 & .328 & .280 \\
Anxious & .202 & .099 & .174 & .128 & .171 & .234 & .087 & .209 & .266 & .214 \\
Confident & .434 & .361 & .424 & .337 & .422 & .498 & .358 & .477 & .575 & .487 \\
Desperate & .285 & .178 & .260 & .218 & .259 & .249 & .252 & .248 & .333 & .252 \\
Frustrated & .472 & .143 & .377 & .508 & .387 & .478 & .403 & .463 & .491 & .465 \\
Happy & .456 & .402 & .471 & .597 & .490 & .508 & .455 & .508 & .523 & .508 \\
Interested & .208 & .179 & .210 & .212 & .207 & .269 & .336 & .295 & .374 & .300 \\
Relaxed & .492 & .529 & .510 & .548 & .515 & .520 & .475 & .516 & .646 & .529 \\
Satisfied & .439 & .351 & .435 & .365 & .428 & .490 & .496 & .499 & .348 & .486 \\
Surprised & .204 & .072 & .179 & .339 & .197 & .284 & .146 & .268 & .327 & .275 \\
\hline
Average & .340 & .244 & .329 & .362 & .333 & .383 & .321 & .377 & .421 & .380 \\
\hline
        
  \end{tabulary}
\end{table*}

==> tables/label_reg_coeffs.tex <==
\begin{table*}[t]
\small
%\tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, \Huge
  \caption{The coefficients of the linear regression (ordinary least squares) for decision fusion of the multimodal prediction of the intensity of the core set affective labels.}
  \label{tab:label-reg-coefs}
  \centering
  
  \begin{tabulary}{1.0\textwidth}{m{0.07\textwidth}|R{0.06\textwidth}R{0.06\textwidth}R{0.06\textwidth}|R{0.06\textwidth}R{0.06\textwidth}R{0.06\textwidth}}

\hline
  \multirow{3}{*}{Label} & \multicolumn{3}{c|}{Traditional Features} & \multicolumn{3}{c}{Deep Representations} \\ \cline{2-7}
 & \multicolumn{1}{c}{Text} & \multicolumn{1}{c}{Audio} & \multicolumn{1}{c|}{Video} & \multicolumn{1}{c}{Text} & \multicolumn{1}{c}{Audio} & \multicolumn{1}{c}{Video}  \\ %\cline{2-4} \cline{6-8}
 & \multicolumn{1}{c}{TF-IDF} & \multicolumn{1}{c}{MFB} & \multicolumn{1}{c|}{FAU} & \multicolumn{1}{c}{BERT} & \multicolumn{1}{c}{W2V2} & \multicolumn{1}{c}{CLIP}  \\ \cline{1-7}
Annoyed & 85.28\,\% & 5.21\,\% & 9.51\,\% & 21.36\,\% & 29.01\,\% & 49.63\,\% \\
Anxious & 86.97\,\% & 7.52\,\% & 5.51\,\% & 20.97\,\% & 27.48\,\% & 51.55\,\% \\
Confident & 88.36\,\% & 3.69\,\% & 7.95\,\% & 33.86\,\% & 31.83\,\% & 34.31\,\% \\
Desperate & 93.24\,\% & 0.44\,\% & 6.31\,\% & 22.15\,\% & 36.87\,\% & 40.98\,\% \\
Frustrated & 85.56\,\% & 5.00\,\% & 9.44\,\% & 6.45\,\% & 43.13\,\% & 50.42\,\% \\
Happy & 87.94\,\% & 3.72\,\% & 8.33\,\% & 18.06\,\% & 34.74\,\% & 47.20\,\% \\
Interested & 82.50\,\% & 7.24\,\% & 10.26\,\% & 39.41\,\% & 15.98\,\% & 44.61\,\% \\
Relaxed & 90.11\,\% & 4.17\,\% & 5.72\,\% & 30.24\,\% & 27.88\,\% & 41.88\,\% \\
Satisfied & 91.40\,\% & 2.19\,\% & 6.40\,\% & 26.54\,\% & 43.71\,\% & 29.74\,\% \\
Surprised & 88.19\,\% & 2.83\,\% & 8.98\,\% & 22.30\,\% & 41.51\,\% & 36.19\,\% \\
\hline
Average & 87.95\,\% & 4.20\,\% & 7.84\,\% & 24.14\,\% & 33.21\,\% & 42.65\,\% \\
\hline

  \end{tabulary}
\end{table*}
